Feature Re-Embedding: Towards Foundation Model-Level Performance in Computational Pathology

Multiple instance learning (MIL) is the most widely used framework in computational pathology, encompassing sub-typing, diagnosis, prognosis, and more. However, the existing MIL paradigm typically requires an offline instance feature extractor, such as a pre-trained ResNet or a foundation model. This approach lacks the capability for feature fine-tuning within the specific downstream tasks, limiting its adaptability and performance. To address this issue, we propose a Re-embedded Regional Transformer (R$^2$T) for re-embedding the instance features online, which captures fine-grained local features and establishes connections across different regions. Unlike existing works that focus on pre-training powerful feature extractor or designing sophisticated instance aggregator, R$^2$T is tailored to re-embed instance features online. It serves as a portable module that can seamlessly integrate into mainstream MIL models. Extensive experimental results on common computational pathology tasks validate that: 1) feature re-embedding improves the performance of MIL models based on ResNet-50 features to the level of foundation model features, and further enhances the performance of foundation model features; 2) the R$^2$T can introduce more significant performance improvements to various MIL models; 3) R$^2$T-MIL, as an R$^2$T-enhanced AB-MIL, outperforms other latest methods by a large margin.The code is available at: https://github.com/DearCaat/RRT-MIL.

==> sec/1.tex <==
\section{Introduction}
\label{sec:intro}
% In the field of computational pathology (CPATH), tissue phenotyping plays a crucial role in determining objective histopathological features present within gigapixel-sized whole slide images (WSIs) for cancer diagnosis~\cite{javed2020intro_1,kather2016intro_2,chen2022hipt,lu2021nature,pinckaers2020intro_pami}.
% However, WSIs, which can be of enormous sizes, ranging from 100 million pixels to 10 billion pixels, is a challenging computer vision domain.
% To address this problem, multiple instance learning (MIL) is usually adopted to take diagnosis analysis as a weakly supervised learning problem~\cite{srinidhi2021survey,maron1997mil_1,dietterich1997mil_2}.
% Under MIL, each slide (WSI), referred to as a bag, is divided into a large number of patches, referred to as instances. Due to the large and variable number of patches per slide, it is infeasible to jointly train an patch feature extraction network with MIL model in an end-to-end manner. Therefore, considering efficiency and feasibility, a offline ResNet-50 (R50) model~\cite{he2016deep}, which pre-trained in ImageNet-1k~\cite{deng2009imagenet}, is often used to extract visual features from the patches. Then input them to the MIL model for slide classification.

\begin{figure}[t]
    \begin{center}
    \includegraphics[width=8.5cm]{./imgs/first_page.pdf}
    \end{center}
    % \caption{Illustration of the proposed MIL paradigm which introduces instance feature re-embedding. We visualize the instance features, where \textcolor{orange}{orange} indicates positive and \textcolor{blue}{blue} indicates negative.}
    \caption{\textbf{Left:} The conventional MIL paradigm lacks fine-tuning of the offline embedded instance features. \textbf{Right:} The proposed MIL paradigm that introduces instance feature re-embedding to provide more discriminative features for the MIL model.}
    \label{fig:intro}
\end{figure}

% Illustration of the pervious MIL and the proposed R$^2$T-MIL paradigms. By re-embedding the instance features, R$^2$T-MIL improves the discriminability of the features compared to previous MIL methods.
% In computational pathology, tissue phenotyping is critical for determining objective histopathological features present within gigapixel-sized whole slide images (WSIs) for cancer diagnosis~\cite{javed2020intro_1,kather2016intro_2,chen2022hipt,lu2021nature,pinckaers2020intro_pami}.
% WSIs can be of enormous sizes, ranging from 100 million pixels to 10 billion pixels. The enormous image size poses bottlenecks to applying deep learning methods for WSI analysis, such as the difficulty of fine-grained annotation and fitting the WSI (slide) into GPU memory. 

% To address the data annotation challenge, weakly supervised learning is usually adopted to model WSI analysis, \textit{i.e.} slide-level labeling is provided as limited supervision. Then the model learning problem is formulated into a multiple instance learning (MIL) task. Under MIL, each slide, referred to as a bag, is divided into a large number of image patches, referred to as instances. 
% As shown in Figure~\ref{fig:intro}(a), many MIL-based WSI classification methods use the following three-stage: 1) slide patching, 2) instance feature extraction, and 3) bag label prediction. 
% Most previous MIL models focus on predicting the bag label with extracted instance features.

% AB-MIL~\cite{ilse2018attention} is among the representative frameworks, which leverages an attention-based operator to aggregate instances features and predict the slide label with the high-level bag representation. 
% There are subsequent works~\cite{li2021dual,shao2021transmil,li2021dt,zhao2022setmil} improve the AB-MIL model by modifying its attention mechanism, such as the TransMIL~\cite{shao2021transmil} that uses the Nystr\"om Multi-head Self-attention (N-MSA) structure~\cite{xiong2021nystromformer}. 

% Though achieving "clinical-grade" performance on many tasks~\cite{chen2022hipt,zhang2022dtfd}, the conventional MIL paradigm has an important design challenge due to the huge instance number.
% Learning the backbone instance feature extractor, instance-level feature aggregator, and bag-level classifier in a holistic end-to-end framework becomes infeasible because of the prohibitive memory cost. Most previous works extract instance features offline with networks pre-trained on natural images~\cite{clam,shao2021transmil,zhang2022dtfd}.
% As shown in Figure~\ref{fig:intro}(a),
% this separation leads to low discriminative features and sub-optimal overall framework performance. 
% To alleviate this issue, some works~\cite{li2021dual,chen2022hipt} utilize self-supervised methods to pre-train feature extractor on a massive amount of WSIs, but this approach is costly. 

% We find that utilizing an online Transformer~\cite{vaswani2017attention} for feature enhancement prior to feature aggregation is a superior and more efficient solution, which we refer to as \textit{feature re-embedding}.
% The new paradigm is illustrated in Figure~\ref{fig:intro}(b).
% However, using existing general Transformer-like MIL structures, like TransMIL~\cite{shao2021transmil}, as a re-embedding module poses significant challenges due to their primary focus on aggregating instance features. 
% The complexity of such structures diminish their efficiency and exacerbate the issue of overfitting. Specifically, the global approximate self-attention, N-MSA~\cite{xiong2021nystromformer}, is the main reason. While it addresses the problem of excessive memory consumption caused by the long sequence length, also incurs a significant cost in efficiency. Furthermore, the features re-embedded through the global self-attention lacks diversity, hindering the aggregation of instance features. Section~\ref{sec:vis} presents more details.

% To better and more efficient re-embed features, we propose a lightweight Re-embedded Regional Transformer, called R$^2$Transformer, which can be learned jointly with other MIL models. 
% R$^2$Transformer only consists of a layer of region-based multi-head self-attention (R-MSA). 
% After dividing instance sequence into multiple regions, R-MSA performs native multi-head self-attention within each region. 
% This approach not only mitigates the excessive computational time and memory consumption caused by self-attention with long sequence inputs, but also re-embeds discriminative features with greater diversity. Additionally, we propose an embedded position encoding generator (EPEG), which can be incorporated into the MSA module and perform position encoding within each region. Compared to existing position encoding strategies, EPEG is more suitable for lightweight R$^2$Transformer.
% The main contributions can be summarized as:

% In computational pathology, tissue phenotyping is critical for determining objective histopathological features present within gigapixel-sized whole slide images (WSIs) for cancer diagnosis~\cite{javed2020intro_1,kather2016intro_2,chen2022hipt,lu2021nature,pinckaers2020intro_pami}.
% WSIs can be of enormous sizes, ranging from 100 million pixels to 10 billion pixels. The enormous image size poses bottlenecks to applying deep learning methods for WSI analysis, such as the difficulty of fine-grained annotation and fitting the WSI (slide) into GPU memory.

% To address the data annotation challenge, weakly supervised learning is usually adopted to model WSI analysis, e.g., slide-level labeling is provided as limited supervision. Then the model learning problem is formulated into a multiple instance learning (MIL) task. Under MIL, each slide, referred to as a bag, is divided into a large number of image patches, referred to as instances.
With the rapid development of digital imaging and scanning technology, the digital slide scanner has become widely used in histopathology, paving the way for digital pathology~\cite{javed2020intro_1,kather2016intro_2,chen2022hipt,lu2021nature,pinckaers2020intro_pami}. In this manner, the entire tissue slide is scanned into a whole slide image (WSI) with ultra-high pixels, which greatly facilitates communication and diagnostic decision-making by pathologists. Nevertheless, pixel-level labeling of ultra-high resolution WSI is time-consuming and labor-intensive, which makes it difficult to classify WSI using existing deep learning techniques accurately. 

To address this problem, multiple instance learning (MIL) is adopted to take WSI classification as a weakly supervised learning problem. MIL divides each slide (called a bag) into a large number of image blocks, referred to as instances.
As shown in Figure~\ref{fig:intro}(a), previous MIL-based WSI classification methods~\cite{clam,ilse2018attention,li2021dual,zhang2022dtfd,shao2021transmil,chen2022hipt} perform the following three-step: 1) instance feature extraction, 2) instance feature aggregation, and 3) bag classification.
% Most previous MIL models focus on predicting the bag label with extracted instance features.
Most previous MIL models focus on the last two steps, where the extracted instance features are utilized to predict the bag label.
AB-MIL~\cite{ilse2018attention} is among the representative frameworks, which leverages an attention-based operator to aggregate instances features and predict the slide label with the high-level bag representation.
Recent works~\cite{li2021dual,shao2021transmil,li2021dt,zhao2022setmil} improve on AB-MIL by modifying its attention mechanism, such as the TransMIL~\cite{shao2021transmil} that uses the Nystr\"om Multi-head Self-attention (N-MSA) structure~\cite{xiong2021nystromformer}.

Though achieving ``clinical-grade" performance on many tasks~\cite{chen2022hipt,zhang2022dtfd}, the conventional MIL paradigm has an important design challenge due to the huge instance number.
Learning the instance feature extractor, instance-level feature aggregator, and bag-level classifier in a holistic end-to-end framework becomes infeasible because of the prohibitive memory cost. Most previous works utilize the off-line feature extractor pretrained on natural images to extract instance features, resulting in lack of feature fine-tuning process~\cite{clam,shao2021transmil,zhang2022dtfd}.
As shown in Figure~\ref{fig:intro}(a),
this results in low discriminative features and sub-optimal overall framework performance.
To mitigate this issue, some works~\cite{li2021dual,chen2022hipt} employ self-supervised methods to pre-train the feature extractor on a massive amount of WSIs.
But this self-supervised fashion entails more time and computational resources.
% But this approach not only requires a huge amount of data but also consumes a lot of computational resources.

Another intuitive way of addressing the aforementioned issue is to re-embed the features with advanced representation learning techniques (e.g., Transformer~\cite{vaswani2017attention}) online prior to feature aggregation, which is omitted by most MIL-based WSI classification approaches.
\textit{We complement this feature re-embedding step into the common paradigm to yield a new MIL paradigm}, as illustrated in Figure~\ref{fig:intro}(b). Recently, Transformer is widely applied for feature aggregation in WSI classification due to its ability to encode the mutual-instance relation~\cite{shao2021transmil,zhang2022dtfd,zhao2022setmil}. As a powerful representation learning method, Transformer is verified as a good re-embedding way in many domains~\cite{chen2022structure,zerveas2021transformer,yang2021graphformers,ge2021revitalizing}. \textbf{\textit{However, directly applying the existing Transformers in WSI classification brings some new problems due to the different design intentions. }} For example, as a representative, TransMIL~\cite{shao2021transmil} employs an approximate global multi-head self-attention named N-MSA~\cite{xiong2021nystromformer} to address the excessive memory consumption issue caused by the overlong sequence input, but incurs a high cost in time efficiency and feature diversity. Moreover, its complex structure also increases the over-fitting risks since the WSI classification scenarios often have fewer training data than the general ones.   

% In this paper, we proposed a novel Transformer-based \textit{feature re-embedding} module to alleviate the problem in WSI classification that the feature extractor cannot be learned with other model components end-to-end. With the initial instance features as input, the re-embedding module learns a more discriminative feature representation for the following MIL model inference use. To address the high computational cost and the low feature diversity challenges caused by current global Transformers, we design a lightweight regional Transformer structure and a new position encoding strategy. The designed module is called Re-embedded Regional Transformer (R$^2$T) in this paper, which can be learned jointly with other MIL models end-to-end.
In this paper, we propose a novel Transformer-based \textit{feature re-embedding} module to alleviate the problem in WSI classification that the feature extractor cannot be learned with other model components end-to-end. With the initial instance features as input, the re-embedding module learns a more discriminative feature representation for the following MIL model. 
% Despite the benefits, 
% Due to the different design intention,
% the current global Transformer is burdened by the high computational cost and the limited feature diversity.
As mentioned above, the existing global Transformer, which is tailored to feature aggregation, suffers from high computational cost and limited feature diversity due to its design intention.
It motivates us to design a lightweight regional Transformer with a new position encoding scheme for feature re-embedding, called Re-embedded Regional Transformer (R$^2$T) and Embedded Position Encoding Generator (EPEG), respectively. R$^2$T can be integrated into mainstream MIL frameworks and trained with the end-to-end manner to fine-tune the pre-extracted offline instance features according to the specific classification task.
% reduce bias caused by the shift between offline feature learning and MIL tasks.
The main contributions can be summarized as follows:
\begin{itemize}
    \item We propose a new paradigm for the MIL model that introduces a re-embedding module to address the problem of poor discriminative ability of instance features caused by offline feature extractors. 
    % We demonstrate the effectiveness and generality of our paradigm through extensive experiments. 
    We demonstrate that feature re-embedding fashion effectively improves MIL models and performs better than the self-supervised pre-training fashion.
    \item We introduce a lightweight regional Transformer for re-embedding instance features. This structure can be plugged into many MIL models, including instance-level MIL, to improve performance further. Combined with AB-MIL, we present the R$^2$T-MIL, which achieves state-of-the-art performance on two common WSI classification benchmarks.
    % Embedded Position Encoding Generator called EPEG
    \item We propose a novel position encoding generator for the lightweight regional Transformer, which combines the advantages of relative position encoding and convolutional position encoding. It can overcome the structural limitations of existing methods and encode local positional information effectively.
    
    % It can be incorporated into the MSA module and utilize a lightweight 1-D convolution to position encoding within each region.
\end{itemize}
% \begin{itemize}
%     \item We propose a new paradigm for the WSI classification that introduces a feature re-embedding module to address the problem of poor discriminative ability of instance features caused by offline feature extractors. 
%     \item We present a lightweight regional Transformer with a new position encoding strategy for re-embedding instance features. It can be plugged into the existing MIL models for end-to-end training to effectively reduce task bias.
%     \item Extensive results on the CAMELYON-16 and TCGA lung cancer datasets demonstrate that R$^2$T can introduce considerable performance improvements to the advanced MIL models and R$^2$T-MIL achieves the state-of-the-art performances in comparison with the recent baselines.
% \end{itemize}



%-------------------------------------------------------------------------
\section{Related Work}
\subsection{Application of MIL in WSI Classification}
% In the WSI classification, MIL methods have a weakly supervised learning paradigm consisting of slide patching, instance feature extraction, and bag label prediction, thanks to outstanding pioneering works~\cite{ilse2018attention,campanella2019clinical,clam}. 
% However, the huge size of WSIs presents a challenge to the instance feature extraction module, which is typically pre-trained on natural image datasets rather than being jointly trained with the bag prediction module.
% Some self-supervised learning-based methods~\cite{chen2022hipt,li2021dual,zhao2020predicting,saillard2021self} attempt to alleviate this bias by pre-training on a large number of WSIs.
% For example, Chen~et al. has adapted DINO~\cite{caron2021dino} to pre-train a vision Transformer~\cite{dosovitskiy2020image} with 10678 gigapixel WSIs~\cite{chen2022hipt}.
% However, they do not explicitly address this bias caused by untunable feature extraction module.
% In this paper, we propose an instance feature re-embedding module that can be jointly trained to directly and efficiently address this issue.

% Many MIL algorithms focus on improve the utilization of extracted instance features for bag prediction. 
% These methods can be divided into two categories: instance-level~\cite{xu2019camel,campanella2019clinical,instance_mil_1,instance_mil_2} and embedding-level~\cite{ilse2018attention,li2021dual,clam,shao2021transmil,zhang2022dtfd,sharma2021cluster,wang2018revisiting}. 
% The former first obtains instance labels and then pools them to obtain the bag label, while the latter aggregates all instance features into a high-level bag embedding, and then obtains the bag prediction. 
% Most embedding-based methods design different attention mechanisms to better aggregate instance features.
% Recently, some works~\cite{shao2021transmil,li2021dt,zhao2022setmil,wang2022lymph} have utilized Transformer blocks~\cite{vaswani2017attention} to aggregate instance information, demonstrating the advantage of self-attention over traditional attention in modeling mutual instance information. 
% In contrast, this paper focuses on re-embedding instance features via Transformer blocks. 
% Similar to our work is HIPT~\cite{chen2022hipt} and SET-MIL~\cite{zhao2022setmil}, which leverage Transformer to update the instance features before aggregation. 
% A key difference is that the re-embedding module proposed in our work can be applied to the complete instance input, rather than being limited to a cropped input sequence due to structural constraints.

% % \vspace{12pt}
% % \noindent\textbf{Efficient Transformer and Position Encoding.}
% \subsection{Efficient Transformer and Position Encoding}
% Transformer~\cite{vaswani2017attention} have emerged as a powerful tool for a broad range of deep learning tasks~\cite{xiong2021nystromformer,dosovitskiy2020image,devlin2018bert,chen2021decision,li2019neural,huang2018music,jaegle2021perceiver}.
% However the quadratic complexity of self-attention on the input sequence length has limited its application to longer sequences (e.g., more than 1000)~\cite{shao2021transmil,xiong2021nystromformer}. 
% In natural language processing (NLP), various works have focused on improving the memory efficiency of the Transformer from different perspective, such as model architecture~\cite{dai2019transformer,michel2019sixteen,lan2019albert}, computational units~\cite{lample2019large,xiong2021nystromformer}, pre-training~\cite{clark2020electra}, sparse representation~\cite{child2019generating}, hash representation~\cite{kitaev2020reformer}.
% % For example, the Nystr\"omformer~\cite{xiong2021nystromformer} adapting the Nystr\"om method to approximate standard self-attention with O(n) complexity. 
% Furthermore, in computer vision, Swin~\cite{liu2021swin} has successfully employed shifted windows to address the efficiency challenges, substantially improving the versatility of vision Transformers. 

% However, for WSI classification, the enormous size of WSI exacerbates the efficiency issues encountered by Transformers,
% making conventional Transformers incapable of processing the entire input sequence~\cite{shao2021transmil}.
% Inspired by the aforementioned methods, we propose a lightweight regional Transformer for instance feature re-embedding. But unlike them, the proposed model is tailored to the intrinsic characteristics of WSI, including variable length of input sequence, limited number of slides, and a small proportion of positive instances.
% Specifically, following~\cite{shao2021transmil}, we use conditional position encoding~\cite{chu2021peg} to adapt variable sequence lengths. But we borrow the idea from relative position encoding~\cite{wu2021irpe,shaw2018self} to embed position encoding in self-attention for facilitating feature re-embedding. 
% In addition, 
% we combines relative position encoding~\cite{wu2021irpe} and conditional position encoding~\cite{chu2021peg} to facilitate feature re-embedding.

MIL-based WSI classification methods generally have a weakly supervised learning paradigm consisting of slide patching, instance feature extraction, and bag label prediction~\cite{ilse2018attention,campanella2019clinical,clam}. 
Due to the huge size of WSIs, the instance features are typically extracted by models pre-trained on natural image datasets.
Some self-supervised learning-based methods~\cite{chen2022hipt,li2021dual,zhao2020predicting,saillard2021self} attempt to alleviate the feature bias by pre-training on a large number of WSIs. For example, Chen~et al. adapted DINO~\cite{caron2021dino} to pre-train a vision Transformer~\cite{dosovitskiy2020image} with more than 10K gigapixel WSIs~\cite{chen2022hipt}. 
% In this paper, we propose an instance feature re-embedding module as a more effective solution.

Extensive efforts are dedicated to the utilization of extracted instance features for bag prediction. 
These methods can be categorized into instance label fusion~\cite{xu2019camel,campanella2019clinical,instance_mil_1,instance_mil_2} and instance feature fusion~\cite{ilse2018attention,li2021dual,clam,shao2021transmil,zhang2022dtfd,sharma2021cluster,wang2018revisiting}. 
Instance label fusion methods first obtain instance labels and then pool them to obtain the bag label, while instance feature fusion methods aggregate all instance features into a high-level bag embedding and then obtain the bag prediction. 
Recently, Transformer blocks~\cite{vaswani2017attention} have been utilized to aggregate instance features~\cite{shao2021transmil,li2021dt,wang2022lymph}, demonstrating the advantage of self-attention over traditional attention~\cite{li2021dual,clam,ilse2018attention} in modeling mutual instance information. 

In contrast, this paper focuses on re-embedding instance features via Transformer before aggregation. 
Similar to our work is SET-MIL~\cite{zhao2022setmil}, which leverages Transformer to update the instance features.
A key difference is that SET-MIL crops the input sequence, resulting in its limited generality, whereas the re-embedding module proposed in this work can be directly applied to complete instance inputs.
% In contrast, this paper focuses on re-embedding instance features via Transformer blocks. 
% Similar to our work is SET-MIL~\cite{zhao2022setmil}, which leverages Transformer to update the instance features. 
% A key difference is that the re-embedding module proposed in our work can be applied to the complete instance input, rather than being limited to a cropped input sequence due to structural constraints.

% \vspace{12pt}
% \noindent\textbf{Efficient Transformer and Position Encoding.}
\subsection{Efficient Transformer and Position Encoding}
Transformer~\cite{vaswani2017attention} have emerged as a powerful tool for a broad range of deep learning tasks~\cite{xiong2021nystromformer,dosovitskiy2020image,devlin2018bert,chen2021decision,li2019neural,huang2018music,jaegle2021perceiver}.
However, the quadratic complexity of self-attention on the input sequence length has limited its application to longer sequences (e.g., more than 1000)~\cite{shao2021transmil,xiong2021nystromformer}. 
In natural language processing, the memory efficiency of the Transformer is improved from multiple perspectives, such as model architecture~\cite{dai2019transformer,michel2019sixteen,lan2019albert}, computational units~\cite{lample2019large,xiong2021nystromformer}, pre-training~\cite{clark2020electra}, sparse representation~\cite{child2019generating}, and hashing representation~\cite{kitaev2020reformer}.
For example, the Nystr\"omformer~\cite{xiong2021nystromformer} adapts the Nystr\"om method to approximate standard self-attention with $O(n)$ complexity. 
In computer vision, Swin Transformer~\cite{liu2021swin} successfully employed shifted windows to address the efficiency challenges, substantially improving the versatility of vision Transformers. Inspired by these methods, we propose a lightweight regional Transformer for instance feature re-embedding. But unlike them, our proposed model is tailored to the intrinsic characteristics of WSI, including the variable length of input sequence, the limited number of slides, and a small proportion of positive instances.

Position encoding is an important component of Transformer~\cite{vaswani2017attention,chu2021peg,wu2021irpe,dosovitskiy2020image,shaw2018rpe}. For instance, Shaw et al. were the first to embed position encoding into MSA to efficiently incorporate relative positional information~\cite{shaw2018rpe}. In the context of MIL, Shao et al. introduced conditional position encoding~\cite{chu2021peg} to handle variable-length sequences and utilized pyramid convolutions to fuse multi-scale positional information~\cite{shao2021transmil}. In this paper, we combine the advantages of these two methods to facilitate feature re-embedding.


%However, for WSI classification, the enormous size of WSI exacerbates the efficiency issues encountered by Transformers,
%making conventional Transformers incapable of processing the entire input sequence~\cite{shao2021transmil}.
% Inspired by the aforementioned methods, we propose a lightweight regional Transformer for instance feature re-embedding. But unlike them, the proposed model is tailored to the intrinsic characteristics of WSI, including variable length of input sequence, limited number of slides, and a small proportion of positive instances.
% Specifically, following~\cite{shao2021transmil}, we use conditional position encoding~\cite{chu2021peg} to adapt variable sequence lengths. But we borrow the idea from relative position encoding~\cite{wu2021irpe,shaw2018self} to embed position encoding in self-attention for facilitating feature re-embedding. 
%------------------------------------------------------------------------- 
\begin{figure*}
\centerline{\includegraphics[width=\textwidth]{./imgs/network.pdf}}
\caption{Overview of proposed R$^2$T-MIL. A set of patches is first cropped from the tissue regions of a slide and embedded in features by an offline extractor. Then, the sequence is processed with the R$^2$T module: (1) squaring of sequence, (2) region partition, and (3) feature re-embedding within each region. Finally, a conventional MIL model predicts the bag labels using the re-embedded instance features.}
\label{fig:model}
\end{figure*}

==> sec/2.tex <==
\section{Methodology}
WSIs are in ultra-high resolution, and the tumor area is only a small proportion of the tissue. These facts hinder the direct classification of the entire WSI. Thus, the WSI is often divided into patches, and the WSI classification issue is solved as a Multiple Instance Learning (MIL) task.

% Our method also belongs to the latter one.
\subsection{Preliminary}
\textcolor{red}{TO DO: simplify this part}

From the perspective of MIL, a WSI $X$ is considered as a bag while its patches are deemed as instances in this bag, which can be represented as $X=\{x_i\}^I_{i=1}$. The instance number $I$ varies for different bags. For a classification task, there exists a known label $Y \in \left \{ 0,1 \right \}$ for a bag and an unknown label $y_i \in \left \{ 0,1 \right \}$ for each of its instances. If there is at least one positive instance in a bag, then this bag is positive; otherwise, it is negative,
\begin{equation}
    Y = \begin{cases}
 0,& \textrm{iff}\,\sum _{i}y_{i} = 0, \\
 1,& \text{otherwise.}
\end{cases}
\end{equation}
% The goal of a MIL model or system $\mathcal{M}(\cdot)$ is to predict the bag label with all instances $\hat{Y}\leftarrow\mathcal{M}(X)$. There are two ways for MIL to accomplish the bag classification. The first way is to predict the instance labels and then aggregate these predictions to obtain the bag label prediction. The second one is to first aggregate instances to yield a bag representation and then classify the bag representation to obtain the final result. Recently, the latter one is more popular due to the recent advance in representation learning. In such a manner, the MIL process can be further divided into three steps: instance feature extraction, instance feature aggregation, and bag classification. The bag labeling process can be defined as follows: 
The goal of a MIL model $\mathcal{M}(\cdot)$ is to predict the bag label with all instances $\hat{Y}\leftarrow\mathcal{M}(X)$.
Following the recent popular approaches~\cite{xu2019camel,instance_mil_2}, the MIL prediction process can be divided into three steps: instance feature extraction, instance feature aggregation, and bag classification. Specifically, this process can be defined as follows:
\begin{equation}
\hat{Y}\leftarrow \mathcal{M}(X):=\mathcal{C}(\mathcal{A}(\mathcal{F}(X))),
\end{equation}
where $\mathcal{F}(\cdot)$, $\mathcal{A}(\cdot)$, and $\mathcal{C}(\cdot)$ are the mapping functions of these aforementioned steps respectively.

% In WSI classification, the bag size is too large due to the high resolution of WSI. Simultaneously extracting all instances requires massive computational resources, which makes the joint optimization of all these three steps in an end-to-end manner pretty difficult. As a rule, most existing MIL-based WSI classification approaches~\cite{clam,zhang2022dtfd,shao2021transmil} adopt a ready-made deep learning model (mostly ResNet-50~\cite{he2016deep}) trained on ImageNet-1k to extract CNN features of patches, and then employ a simple linear projection or MLP to process these features again to yield the instance representations. In such a regime, only the aggregation and classification steps are optimized. However, the inconsistency in the optimization goal between the feature extraction step and the subsequent steps results in a task shift in feature space and degrades WSI classification performance. A direct way to alleviate this problem is by re-embedding on the basis of the extracted instance features. However, most of the existing approaches pay more attention to feature aggregation while omitting the importance of re-embedding. In this paper, we elaborate on the Re-embedded Regional Transformer for addressing this issue and reveal the importance of instance re-embedding in WSI classification. Specifically, our approach includes a re-embedding step after the instance feature extraction and updates the bag labeling process as follows,
% In WSI classification, extracting all instances in a bag requires massive computational resources, which makes the joint optimization of all these three steps in an end-to-end manner pretty difficult. 
% \subsection{}
In WSI classification, extracting all instances in a bag poses a huge computational challenge for end-to-end optimization of these three steps.
Therefore, most existing MIL-based WSI classification approaches~\cite{clam,zhang2022dtfd,shao2021transmil} typically rely on a pre-trained deep learning model (mostly ResNet-50~\cite{he2016deep}) on ImageNet-1k to obtain instance features first. 
Then, they only optimize the aggregation and classification steps. 
However, the inconsistency in the optimization goal between the feature extraction and the subsequent steps results in a task shift in feature space and degrades WSI classification performance. 
An intuitive way to address this problem is by re-embedding based on the extracted instance features, 
while most of the existing approaches pay more attention to feature aggregation and neglect the importance of re-embedding. 
% Currently, most existing methods, most of which use feature aggregation to optimize offline features, ignore instance re-embedding as a crucial optimization approach to enhance the discriminability of instance representation.
In this paper, we elaborate on the Re-embedded Regional Transformer to reveal the importance of instance re-embedding in WSI classification. Specifically, our approach includes a re-embedding step after the instance feature extraction and updates the bag labeling process as follows,
\begin{equation}
\hat{Y}\leftarrow \mathcal{M}(X):=\mathcal{C}(\mathcal{A}(\mathcal{R}(\mathcal{F}(X)))),
\end{equation}
where $\mathcal{R}(\cdot)$ is the mapping function of the re-embedding.


%There are two solutions, one is to assign each instance the bag label and accordingly train a classifier, and then apply the max or average pooling operation on the individual instance classifications to obtain the bag-level results. Another is to learn a bag representation $B$ from the extracted features of instance $H = \left \{ h_1,h_2,\cdots,h_K \right \} $ in a bag, and train a classifier $C(\cdot)$ to perform bag classification $\hat{Y} = C(B)$. This strategy is proven to be more efficient, which referred to as bag embedding-based MIL.
%The bag embedding $B$ is formulated as,
%\begin{equation}
%B = G\left ( \left \{ h_k \mid k = 1,2,\cdots,K  \right \} \right ),
%\end{equation}
%where $G(\cdot)$ represents feature aggregation function, $h_k \in \mathbb{R} ^{D}$ is the extracted feature for instance $k$.


%-------------------------------------------------------------------------
% The application of MIL models in WSI classification faces many challenges due to the ultra-high resolution of WSIs. The biggest challenge is that the large number of instances $K$ makes it difficult for MIL models to undergo end-to-end training, like traditional deep learning models. Typically, the training of embedded MIL models for WSI classification is divided into two stages: pre-training of instance visual feature extractors and training of instance feature-based aggregation and classification models. In this paper, we refer to the latter stage as the training of the embedded MIL model. For the first stage, although there are many outstanding works based on self-supervised learning that try to use WSI images for pre-training, this pre-training is very costly and has not been widely used.

%\subsection{Re-embedded Regional Transformer}
% The application of MIL models in WSI classification faces many challenges due to the ultra-high resolution of WSIs. The biggest challenge is that the large number of instances $K$ makes it difficult for MIL models to undergo end-to-end training, like traditional deep learning models.
% Therefore, many existing outstanding works use a offline classification model (usually ResNet-50) trained on ImageNet-1k~\cite{deng2009imagenet} as the instance visual feature extractor $f$. The instance feature extraction is formulated as,
%\begin{equation}
%    H = p\left ( f\left ( \left \{ x_k \mid k = 1,2,\cdots,K  \right \} \right ) \right ),
%\end{equation}
%where $p$ is a lightweight projection head with only one linear layer, and the feature extractor $f$ is not learnable. With $f$, existing embedded MIL models are formed into the paradigm of "offline embedding-dimension projection-feature aggregation-classification", which can be formulated as,
%\begin{equation}
%    \hat{Y} = C\left ( B\left ( p\left ( f\left ( X \right ) \right ) \right ) \right ).
%\end{equation}
%To address the challenge of poor discriminative ability of instance features caused by the untrainable feature extractor, we propose the re-embedding module $R\left ( \cdot \right )$. It leverages the Transformer architecture to re-embed instance features, enabling end-to-end optimization with the MIL model.This leads to the production of more discriminative features. The new paradigm "offline embedding - dimension projection - {\color{blue}feature re-embedding} - feature aggregation - classification" is proposed to accommodate the incorporation of re-embedding module. This can be formulated as,
%\begin{equation}
%    \hat{Y} = C\left ( B\left ( {\color{blue}\boldsymbol{R} }\left ( p\left ( f\left ( X \right ) \right ) \right ) \right ) \right ).
%\end{equation}
%% The key component of the model is the Re-Embedding module, which leverages the Transformer architecture to re-embed instance features.
%
%Based on this new paradigm, we propose the R$^2$T-MIL model.
%The R$^2$T-MIL includes a lightweight local Transformer, referred to as Lformer, which enables efficient modeling of local inter-instance relationships, resulting in rapid and effective re-embedding of instance features. Additionally, the R$^2$T-MIL model incorporates an Efficient Position Encoding Generator (EPEG) that encodes positional information of instances without compromising computational efficiency.
%By incorporating a classical Attention-based feature aggregation module, the R$^2$T-MIL model can performing binary classification and subclass classification tasks in WSI analysis. Figure~\ref{fig:model} shows the overview of the R$^2$T-MIL, and its components will be described in the following sections.

%-------------------------------------------------------------------------
\subsection{Re-embedded Regional Transformer}
We propose a lightweight Transformer named Re-embedded Regional Transformer (R$^2$Transformer, R$^2$T) to re-embed the input instance features as the new instance representations,
\begin{equation}
    Z= \{z_i\}_{i=1}^I:=\mathcal{R}(H)\in \mathbb{R}^{I\times D},
\end{equation}
where $\mathcal{R}(\cdot)$ is the mapping function of the R$^2$Transformer here, $H=\{h_i\}_{i=1}^I:=\mathcal{F}(X)\in \mathbb{R}^{I\times D}$ is the processed input instance features, and $z_i=\mathcal{R}(h_i)$ is the new embedding of the $i$-th instance. $D$ is the dimensionality of the embedding. The R$^2$Transformer can be flexibly plugged into the MIL framework as a re-embedding module after feature input and before instance aggregation to reduce bias caused by the shift between offline feature learning and MIL tasks. The whole re-embedding process in the R$^2$Transformer can be formulated as,
\begin{equation}
    \mathcal{R}\left ( H \right ) := \textrm{R-MSA}\left ( \textrm{LN}\left ( H \right ) \right ) + H,
\end{equation}
where R-MSA$(\cdot)$ denotes Regional Multi-head Self-attention, and LN$(\cdot)$ denotes Layer Normalization~\cite{ba2016layernorm}.
 % of $\left ( \left \lceil \sqrt{K}  \right \rceil\times \left \lceil \sqrt{K}  \right \rceil \right )$

\noindent\textbf{Regional Multi-head Self-attention:}
Since instance number $I$ is very large, most Transformers in the WSI classification commonly adopt two strategies to avoid self-attention computation for all instances. The first method is to sample or aggregate the original large instance set into a small one, after which global self-attention is performed~\cite{li2021dt,zhao2022setmil}.  The second method performs the Nystrom algorithm~\cite{xiong2021nystromformer} to approximate the global self-attention~\cite{shao2021transmil}. Although these methods address the scalability issue of self-attention with a large $I$, they omit the property that the tumor areas are local and represent a small part of the whole image. Performing global self-attention on all instances results in feature homogenization. Moreover, different from the conventional MIL application scenarios, the instances in each bag have ordinal relations in WSI classification due to the fact that they are all collected from the same slide in order. These facts motivate us to design the Regional Multi-head Self-attention (R-MSA) that blocks the bag into several different regions and performs self-attention in each region separately. R-MSA takes into account the aforementioned WSI properties and makes use of instance ordinal relation information to reduce computation complexity and highlight salient local features. 

Figure~\ref{fig:model} shows the basic structure of R-MSA. In R-MSA, the input instance features are reshaped into a 2-D feature map, $ H \in \mathbb{R}^{I \times D} \rightarrow H \in \mathbb{R}^{\left \lceil \sqrt{I}  \right \rceil\times \left \lceil \sqrt{I}  \right \rceil \times D} $. And $L \times L$ regions are then divided evenly across the map in a non-overlapping manner, with each containing $M \times M$ instances where $L\times M= \lceil\sqrt{I}\rceil$.~\footnote{To make the number of regions $\left ( L,L \right )$ divisible by the feature map size, zero padding is employed on the feature map if needed.} For example, the region partition starts from the top-left instance, and an $8 \times 8$ feature map is evenly partitioned into $2 \times 2$ regions of size $4 \times 4 \left ( L=2, M=4 \right )$. In this paper, \textit{we fixe the number of regions $L$ rather than the size of regions $M$ to obtain $L \times L$ regions with adaptive size.} By default, $L$ is set to $8$.

Self-attention is computed within each local region, and the 2-D feature map is finally flattened and reshaped back to its original shape. The whole process of R-MSA can be denoted as,
% \begin{matrix}
% % H \in \mathbb{R}^{\left \lceil \sqrt{K}  \right \rceil\times \left \lceil \sqrt{K}  \right \rceil \times D} \leftarrow H \in \mathbb{R}^{K \times D}, \\
% H \in  \mathbb{R}^{L\times M\times M \times D} \leftarrow H \in \mathbb{R}^{K \times D},\\
% \hat{H}^{l} =  \textrm{MSA}\left (  H^{l}  \right ),H = \left \{ H^{1},\cdots,H^{L} \right \},\\
% % \hat{H}\in \mathbb{R}^{L\times M \times M \times D} \leftarrow \textrm{Concat}\left ( \hat{H}^{1},\cdots,\hat{H}^{L} \right ),\\
% \hat{H}\in \mathbb{R}^{K \times D}\leftarrow \hat{H}\in \mathbb{R}^{L\times M \times M \times D},\\
% \end{matrix}
\begin{equation}
\begin{aligned}
&\bm{Step~1:}~  H \in \mathbb{R}^{I \times D}\overset{\textrm{Squaring}}\longrightarrow H \in  \mathbb{R}^{L^2\times M^2 \times D}, \\
&\bm{Step~2:}~ H\overset{\textrm{Partition}}\longrightarrow \{H^l\}^{L^2}_{l=1}, H^l\in  \mathbb{R}^{M\times M \times D},\\
&\bm{Step~3:}~
Z:=\{Z^l\}^{L^2}_{l=1},Z^l=\mathcal{S}(H^l)\in  \mathbb{R}^{M\times M \times D},\\
%\hat{H}\in \mathbb{R}^{L^2\times M^2 \times D} \leftarrow \textrm{Concat}\left ( \hat{H}^{1},\cdots,\hat{H}^{L^2} \right ),\\
&\bm{Step~4:}~Z\in \mathbb{R}^{L^2\times M^2 \times D}\overset{\textrm{Flatten}}\longrightarrow Z\in \mathbb{R}^{I \times D},\\
\end{aligned}
\end{equation}
where $\mathcal{S}(\cdot)$ is vanilla multi-head self-attention with our proposed Embedded Position Encoding Generator (EPEG).

\begin{figure}[t]
    \centering
    \includegraphics[width=8.0cm]{./imgs/epeg.pdf}
    \caption{Illustration of Embedded Position Encoding Generator. }
    \label{fig:epeg}
\end{figure}

\begin{table*}[t]
\small
\centering
% \setlength{\tabcolsep}{4pt}
\begin{tabular}{llccccccc}
\toprule
\multicolumn{2}{c}{\multirow{2}{*}{Methods }}        & \multicolumn{3}{c}{CAMELYON-16}   && \multicolumn{3}{c}{TCGA-BRCA}  \\ \cline{3-5} \cline{7-9}
                                 && \makecell[c]{Accuracy}           & \makecell[c]{AUC}      & \makecell[c]{F1-score}
                                 && \makecell[c]{Accuracy}          & \makecell[c]{AUC}      & \makecell[c]{F1-score}   \\ \midrule

\multirow{8}{*}{\rotatebox{90}{\makecell[c]{ResNet-50\\ImageNet pretrained}}}&AB-MIL~\cite{ilse2018attention}  & 90.06$\pm$0.60             & 94.00$\pm$0.83           & 87.40$\pm$1.05
                                 && 87.72$\pm$0.63            & 93.14$\pm$0.33           & 87.10$\pm$0.71         \\
&CLAM~\cite{clam}        & 90.14$\pm$0.85              & 94.70$\pm$0.76               & 88.10$\pm$0.63
                                 && 85.17$\pm$0.03& 91.67$\pm$0.02& 70.68$\pm$0.04   \\
&DSMIL~\cite{li2021dual}          & 90.17$\pm$1.02             & 94.57$\pm$0.40           & 87.65$\pm$1.18                                 && 87.68$\pm$0.03  & 92.12$\pm$0.02         & 74.25$\pm$0.04 \\
&TransMIL~\cite{shao2021transmil} & 89.22$\pm$2.32              & 93.51$\pm$2.13   & 85.10$\pm$4.33
                                 && 85.15$\pm$0.03              & 91.38$\pm$0.02             & 70.9$\pm$0.04  \\
&DTFD-MIL~\cite{zhang2022dtfd}    & 90.22$\pm$0.36              &  95.15$\pm$0.14           & 87.62$\pm$0.59
                                 && \underline{88.46$\pm$0.43}              & \underline{91.55$\pm$0.15}             & 87.92$\pm$0.36  \\
&IBMIL~\cite{lin2023interventional}    & 91.23$\pm$0.41              &  94.80$\pm$1.03           &88.80$\pm$0.89
                                 && 88.36$\pm$0.28              & 93.60$\pm$0.06             & \underline{88.16$\pm$0.59}  \\
&MHIM-MIL~\cite{tang2023mhim}    & \underline{91.81$\pm$0.82}              &  \underline{96.14$\pm$0.52}           & \underline{89.94$\pm$0.70}
                                 && 83.90$\pm$3.38              & 92.48$\pm$1.38& \underline{69.91$\pm$3.76}  \\
& \rowcolor{dino}
 \textbf{R$^2$T-MIL}        & \textbf{92.40$\pm$0.31}     & \textbf{97.32$\pm$0.29}      & \textbf{90.63$\pm$0.45}
                                && \textbf{88.33$\pm$0.67}& \textbf{93.17$\pm$1.45}& \textbf{ 75.02$\pm$1.58}\\
\midrule
\multirow{8}{*}{\rotatebox{90}{\makecell[c]{PLIP\\WSI pretrained}}}&AB-MIL~\cite{ilse2018attention}  & 90.06$\pm$0.60             & 94.00$\pm$0.83           & 87.40$\pm$1.05
                                 && 87.72$\pm$0.63            & 93.14$\pm$0.33           & 87.10$\pm$0.71         \\
&CLAM~\cite{clam}        & 90.14$\pm$0.85              & 94.70$\pm$0.76               & 88.10$\pm$0.63
                                 && 88.07$\pm$0.49             & 93.47$\pm$0.16            & 87.61$\pm$0.52   \\
&DSMIL~\cite{li2021dual}          & 90.17$\pm$1.02             & 94.57$\pm$0.40           & 87.65$\pm$1.18                                 && 88.42$\pm$0.10  & 93.72$\pm$0.22         & 87.93$\pm$0.09 \\
&TransMIL~\cite{shao2021transmil} & 89.22$\pm$2.32              & 93.51$\pm$2.13   & 85.10$\pm$4.33
                                 && 86.39$\pm$0.98              & 92.02$\pm$0.98             & 86.06$\pm$0.98  \\
&DTFD-MIL~\cite{zhang2022dtfd}    & 90.22$\pm$0.36              &  \underline{95.15$\pm$0.14}           & 87.62$\pm$0.59
                                 && \underline{88.46$\pm$0.43}              & \underline{93.78$\pm$0.15}             & 87.92$\pm$0.36  \\
&IBMIL~\cite{lin2023interventional}    & \underline{91.23$\pm$0.41}              &  94.80$\pm$1.03           & \underline{88.80$\pm$0.89}
                                 && 88.36$\pm$0.28              & 93.60$\pm$0.06             & \underline{88.16$\pm$0.59}  \\
&MHIM-MIL~\cite{tang2023mhim}    & \underline{91.23$\pm$0.41}              &  97.79$\pm$1.03           & \underline{88.80$\pm$0.89}
                                 && 88.36$\pm$0.28              & 93.60$\pm$0.06             & \underline{88.16$\pm$0.59}  \\
& \rowcolor{dino}
 \textbf{R$^2$T-MIL}        & \textbf{92.40$\pm$0.31}     & \textbf{98.05$\pm$0.29}      & \textbf{90.63$\pm$0.45}
                                && \textbf{89.37$\pm$0.56} & \textbf{94.82$\pm$0.03} & \textbf{88.89$\pm$0.72} \\

\bottomrule
\end{tabular}
\caption{The performance of different MIL approaches on CAMELYON-16 and TCGA Lung Cancer. The highest performance is in bold, and the second-best performance is underlined. 
The Accuracy and F1-score are determined by the optimal threshold.
}
\label{tab:main_comp}
\end{table*}

\noindent\textbf{Embedded Position Encoding Generator:}
Following~\cite{shao2021transmil,chu2021peg}, we adopt a convolutional computation called Position Encoding Generator (PEG) to address the challenge of traditional position encoding strategies being unable to handle input sequences of variable length.
% Inspired by the relative position encoding strategy~\cite{wu2021irpe,liu2021swin}, we embed the PEG into R-MSA to eliminate the restriction of MSA layers, which imposed by the conventional apporths.  However, unlike~\cite{shao2021transmil}, the EPEG can encode using a more lightweight 1-D convolution $\textrm{Conv}_{\textrm{1-D}}(\cdot)$ since it is embedded within the MSA module. 
However, these methods are designed for multi-layered global MSA and unsuitable for the single-layered regional R$^2$Transformer. To address this issue, we propose a novel approach called Embedded PEG (EPEG) by incorporating PEG into the R-MSA module, inspired by the relative position encoding strategy~\cite{wu2021irpe,liu2021swin,shaw2018rpe}. By embedding the PEG into the MSA module, EPEG can utilize a lightweight 1-D convolution $\textrm{Conv}_{\textrm{1-D}}(\cdot)$ to encode in each region separately.
The structure of EPEG is shown in Figure~\ref{fig:epeg}. Take the instances in the $l$-th region as an example, and the EPEG can be formulated as,
\begin{equation}
\alpha_{ij}^{l} = \textrm{softmax} \left ( e_{ij}^{l} {\color{blue} + \textrm{Conv}_{\textrm{1-D}}\left ( e_{ij}^{l} \right ) } \right ),
\end{equation}
where $\alpha_{ij}^{l}$ is the attention weight of $H^{l}_{j}$ with respect to $H^{l}_{i}$, and $e_{ij}^{l}$ is calculated using a scaled dot-product attention:
\begin{equation}
    e_{ij}^{l} = \frac{\left ( H^{l}_{i}W^{Q} \right ) \left ( H^{l}_{j}W^{K} \right )^{T}}{\sqrt{D}},
\end{equation}
where $H^{l}_{i}$ is the $i$-th instance features in $l$-the region $H^l$.
With EPEG, the R-MSA can be further represented as,
\begin{equation}
    \begin{aligned}
&\textrm{R-SA} = \sum_{j=1}^{M\times M}\alpha_{ij}^{l} \left ( H^{l}_{j}W^{V} \right ),\\
&\textrm{R-MSA} = \textrm{Concat}\left ( \textrm{R-SA}_1,\cdots,\textrm{R-SA}_{N_{head}} \right )W^O
\end{aligned}
\end{equation}
where the projections $W^{Q}$, $W^{K}$, $W^{V}$, and $W^{O}$ are parameter matrices sharing across the regions. The $N_{head}$ denotes the number of heads.


\subsection{R$^2$Transformer-based MIL}
Once we obtain the re-embedding of instances, any instance aggregation method and classifier can be applied to accomplish the WSI classification. The re-embedding $\mathcal{R}(\cdot)$ will be optimized with the instance aggregation module $\mathcal{A}(\cdot)$ and the bag classifier $\mathcal{C}(\cdot)$ together, 
\begin{equation}
    \{\mathcal{\hat{R}},\mathcal{\hat{A}},\mathcal{\hat{C}}\}\leftarrow \arg\min L(Y,\hat{Y})=L(Y,\mathcal{C}(\mathcal{A}(\mathcal{R}(H)))),
\end{equation}
where $L(\cdot,\cdot)$ represents any MIL loss. If there is no special declaration, we adopt the instance aggregation method and the bag classifier of AB-MIL~\cite{ilse2018attention} by default.
